MPC-based Motion Planning for Autonomous Truck-Trailer Maneuvering

Time-optimal motion planning of autonomous vehicles in complex environments is a highly researched topic. This paper describes a novel approach to optimize and execute locally feasible trajectories for the maneuvering of a truck-trailer Autonomous Mobile Robot (AMR), by dividing the environment in a sequence or route of freely accessible overlapping corridors. Multi-stage optimal control generates local trajectories through advancing subsets of this route. To cope with the advancing subsets and changing environments, the optimal control problem is solved online with a receding horizon in a Model Predictive Control (MPC) fashion with an improved update strategy. This strategy seamlessly integrates the computationally expensive MPC updates with a low-cost feedback controller for trajectory tracking, for disturbance rejection, and for stabilization of the unstable kinematics of the reversing truck-trailer AMR. This methodology is implemented in a flexible software framework for an effortless transition from offline simulations to deployment of experiments. An experimental setup showcasing the truck-trailer AMR performing two reverse parking maneuvers validates the presented method.

==> results-discussion.tex <==
% !TeX root = paper.tex
\section{Experimental Results and Discussion}
\label{results}
The performance of the presented approach is evaluated experimentally as described in the previous section. 

Bastiaan

- show the traveled trajectory\\
- tracking accuracy\\
- rekentijden

\begin{figure}
    % \centering
    \includegraphics[width=0.6\linewidth]{figures/tracking_error.pdf}
    \caption{Euclidean norm of the tracking error.}
    \label{fig:tracking_error}
\end{figure}
